Masked Autoencoders as Universal Speech Enhancer

Supervised speech enhancement methods have been very successful. However, in practical scenarios, there is a lack of clean speech, and self-supervised learning-based (SSL) speech enhancement methods that offer comparable enhancement performance and can be applied to other speech-related downstream applications are desired. In this work, we develop a masked autoencoder based universal speech enhancer that is agnostic to the type of distortion affecting speech, can handle multiple distortions simultaneously, and is trained in a self-supervised manner. An augmentation stack adds further distortions to the noisy input data. The masked autoencoder model learns to remove the added distortions along with reconstructing the masked regions of the spectrogram during pre-training. The pre-trained embeddings are then used by fine-tuning models trained on a small amount of paired data for specific downstream tasks. We evaluate the pre-trained features for denoising and dereverberation downstream tasks. We explore different augmentations (like single or multi-speaker) in the pre-training augmentation stack and the effect of different noisy input feature representations (like $log1p$ compression) on pre-trained embeddings and downstream fine-tuning enhancement performance. We show that the proposed method not only outperforms the baseline but also achieves state-of-the-art performance for both in-domain and out-of-domain evaluation datasets.

==> new/README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)


Carried on CTAN only, for non-IEEE related work:

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

EEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************


==> tex/rebuttal.tex <==
%\section{Rebuttal}
We address some of the primary concerns of reviewers.

\section{Reviewer 1}
\begin{itemize}
    \item[(1)] \textbf{Comment:} \textit{The proposed method is compared to state-of-the-art approaches, but the comparison is not entirely fair. The model is trained on the LibriSpeech dataset in a self-supervised manner, then fine-tuned and tested on the Valentini dataset, unlike the other approaches it’s compared to. Consequently, Table 1 does not provide a fair comparison, and aligning the setup more closely with that of the methods being compared would be beneficial.}\\


    \textbf{Response:} Main novelty of our work is to demonstrate how a self-supervised learning (SSL) based approach can be a universal speech enhancer by handling a number of downstream enhancement tasks like denoising, dereverberation, background babble removal, etc. To achieve this we propose a novel pretraining scheme using an extensive augmentation stack. Since our approach is SSL-based, in Table 1, we compare our work against the closest SOTA SSL baselines - AudioMAE for restoration \cite{zhong2023extending} and Boosting SSL \cite{hung2022boosting}. This is a fair comparison as both baselines use LibriSpeech for pre-training and Valentini for fine-tuning. The results reinforce our claim.\\

    Table 1 also provides comparisons against several non-SSL methods like DCUNet \cite{choi2018phase}, SGMSE+ \cite{richter2023speech}, UNIVERSE \cite{serra2022universal}, etc to demonstrate that our method is competitive with non-SSL SOTA discriminative and generative approaches as well. Since these methods are not SSL-based, there is no concept of pre-training. As noted by reviewer \#4 in their comment \textit{"The authors have compared their approach with a number of state of the art methods using multiple metrics. While the extent of the experiments and the comparison is quite nice"}, we aimed to highlight how our work stacks up against current research in the wider speech enhancement space. \\

    

    \item[(2)] \textbf{Comment:} \textit{In Table 2 (zero-shot speech enhancement), notable methods such as DCUNET and SSL boosting are missing. It’s unfortunate they aren’t included, as these approaches are known to perform well in zero-shot scenarios.}\\


    \textbf{Response:} There are no published numbers on DAPS dataset for DCUNet and SSL Boosting, for us to be able to include in our paper. Both papers only reported results on the Valentini test set that we included in Table 1.  \\
    
    SSL-based methods are well-known to have better generalization ability hence we compared our work to the current SOTA SSL method, AudioMAE for restoration \cite{zhong2023extending}. In keeping with the motivation for Table 1, we also offer comparisons with non-SSL works like SGMSE+ \cite{richter2023speech}, UNIVERSE \cite{serra2022universal}, etc, which have published numbers on DAPS. \\
    
    Our main aim in Table 2 was to supplement the in-domain performance already established in Table 1 (for many methods) with out-of-domain generalization performance. It would be infeasible to consider all possible enhancement models in the literature hence we restricted ourselves to our closest baseline and a few popular works that have officially reported numbers on the DAPS dataset. \\  

\section{Reviewer 2}

We thank the reviewer for appreciating our work by providing a \textit{Definite Accept} overall evaluation. We will include the suggested wording changes in our camera-ready version if accepted.

\section{Reviewer 4}
    \item[(3)] \textbf{Comment:} \textit{The results are not very conclusive with different methods being better at different metrics (particularly for the out-of-domain results).}\\

    \textbf{Response:} Diffusion models like SGMSE+ \cite{richter2023speech} usually offer SOTA performance for non-intrusive metrics like NISQA as they excel at generating speech with good human perceptual qualities but do not perform as well at distortion removal as evidenced by their performance for intrusive metrics that require clean reference like PESQ. Moreover, in the case of out-of-domain generalization, our method outperforms SGMSE+ (considered one of the SOTA zero-shot models) on all intrusive metrics except CSIG.

    
\end{itemize}
